Rigorous solution of a Hubbard model extended by nearest-neighbor Coulomb and isotropic exchange interaction on a triangle and tetrahedron

In the preprint cond-mat/0701060 we detected a factor two error in the coding of the Heisenberg term of the Hamiltonian. In the result the exchange term used in the paper was that of an anisotropic Heisenberg model with $J_x=J_y=J$ and $J_z=J/2$. Thus all results given for which J=0 was chosen, remain unchanged, whereas all results containing the exchange parameter remain true for the extended Hubbard model with anisotropic exchange. That model is of some interest by itself, due to the relation to the XXZ model. The differing results for isotropic exchange are given here.

==> figure01d_isotrop.tex <==
\begin{figure}
 \begin{minipage}[t]{0.48\textwidth} 
 \centering 
 \includegraphics[height=55mm]{./canonicalTriangleGsU4JWN2c.eps}\\[1ex]
 \includegraphics[height=55mm]{./canonicalTriangleGsU4JWN4c.eps}\\[1ex]
 \end{minipage} 
 \hfil
 \begin{minipage}[t]{0.48\textwidth}
 \includegraphics[height=55mm]{./canonicalTriangleGsU4JWN3c.eps}\\[1ex]
 \vfil
 \includegraphics[width=55mm]{./canonicalPalette3Site.eps}\\[1ex]
 \end{minipage} 
 \caption{The ground states for the complete $J$-$W$-plane 
  (scaled to primed values) for $U/t=4$, $h/t=0$ and $N=2$ (upper left),
  $N=3$ (upper right), and $N=4$ (down left) respectively.
  Down-right: The palette used here and in Figs. 
  \ref{primedewsTriangleU}-\ref{primedewsTriangleW}
  %the pictures above 
  to indicate the
  irreducible representation (colour) and the maximum $\opS_z$ eigenvalue (intensity)
  of the ground states.}
\label{primedewsTriangleJW}
\end{figure}


==> tetra_abbreviations.tex <==
%\documentclass[a4paper,fleqn]{scrartcl}
%\pagestyle{empty}
%\input{/home/schumann/TEX/mycommands}
%\begin{document}
\parindent0cm
\subsection*{ List of abbreviations }
\beq 
A_1 &=& 9 J^2+36 t J+24 U J-24 W J+768 t^2+16 U^2+16 W^2+48 t U-48 t W-32 U W
 \nonumber \\
A_2 &=& 9 J^2+24 U J-24 W J+256 t^2+16 U^2+16 W^2-32 U W
 \nonumber \\
A_3 &=& 9 J^2+24 U J-24 W J+768 t^2+16 U^2+16 W^2-32 U W
 \nonumber \\
A_4 &=& 9 J^2+24 U J-24 W J+1024 t^2+16 U^2+16 W^2-32 U W
 \nonumber \\
A_5 &=& 27 J^2+72 U J-72 W J+768 t^2+48 U^2+48 W^2-96 U W
 \nonumber \\
A_6 &=& 9 J^2+48 t J+24 U J-24 W J+256 t^2+16 U^2+16 W^2+64 t U-64 t W-32 U W
 \nonumber \\
A_7 &=& 9 J^2+96 t J+24 U J-24 W J+1024 t^2+16 U^2+16 W^2+128 t U-128 t W-32 U W
 \nonumber \\
A_8 &=& 9 J^2-48 t J+24 U J-24 W J+256 t^2+16 U^2+16 W^2-64 t U+64 t W-32 U W
 \nonumber \\
A_9 &=& 3 J-16 t-4 U-4 W
 \nonumber \\
A_{10} &=& 9 J^2-36 t J+24 U J-24 W J+768 t^2+16 U^2+16 W^2-48 t U+48 t W-32 U W
 \nonumber \\
A_{11} &=& 3 J+12 t-20 U-100 W+2 \cos \left(\theta _1\right) \sqrt{A_1}
 \nonumber \\
A_{12} &=& -\frac{J}{4}-t+\frac{5 U}{3}+\frac{25 W}{3}+\frac{1}{12} \cos \left(\theta _1\right) \sqrt{A_1}-\frac{\sin \left(\theta _1\right) \sqrt{A_1}}{4 \sqrt{3}}
 \nonumber \\
A_{13} &=& -\frac{J}{4}-t+\frac{5 U}{3}+\frac{25 W}{3}+\frac{1}{12} \cos \left(\theta _1\right) \sqrt{A_1}+\frac{\sin \left(\theta _1\right) \sqrt{A_1}}{4 \sqrt{3}}
 \nonumber \\
A_{14} &=& -\frac{3 J}{4}+U+5 W+\frac{\cos \left(\theta _2\right) \sqrt{A_2}}{4 \sqrt{3}}-\frac{1}{4} \sin \left(\theta _2\right) \sqrt{A_2}
 \nonumber \\
A_{15} &=& -\frac{3 J}{4}+U+5 W+\frac{\cos \left(\theta _2\right) \sqrt{A_2}}{4 \sqrt{3}}+\frac{1}{4} \sin \left(\theta _2\right) \sqrt{A_2}
 \nonumber \\
A_{16} &=& 3 J-8 U-28 W+\cos \left(\theta _3\right) \sqrt{A_3}
 \nonumber \\
A_{17} &=& -4 U-32 W+\cos \left(\theta _4\right) \sqrt{A_3}
 \nonumber \\
A_{18} &=& -\frac{J}{2}+\frac{4 U}{3}+\frac{14 W}{3}+\frac{1}{12} \cos \left(\theta _3\right) \sqrt{A_3}-\frac{\sin \left(\theta _3\right) \sqrt{A_3}}{4 \sqrt{3}}
 \nonumber \\
A_{19} &=& -\frac{J}{2}+\frac{4 U}{3}+\frac{14 W}{3}+\frac{1}{12} \cos \left(\theta _3\right) \sqrt{A_3}+\frac{\sin \left(\theta _3\right) \sqrt{A_3}}{4 \sqrt{3}}
 \nonumber \\
A_{20} &=& \frac{2 U}{3}+\frac{16 W}{3}+\frac{1}{12} \cos \left(\theta _4\right) \sqrt{A_3}-\frac{\sin \left(\theta _4\right) \sqrt{A_3}}{4 \sqrt{3}}
 \nonumber \\
A_{21} &=& \frac{2 U}{3}+\frac{16 W}{3}+\frac{1}{12} \cos \left(\theta _4\right) \sqrt{A_3}+\frac{\sin \left(\theta _4\right) \sqrt{A_3}}{4 \sqrt{3}}
 \nonumber \\
A_{22} &=& 9 J-12 U-60 W+2 \cos \left(\theta _2\right) \sqrt{A_5}
 \nonumber \\
A_{23} &=& 768 t^2-256 U t+A_9^2+48 J U-64 U W
 \nonumber \\
A_{24} &=& 3 J-12 t-8 U-28 W+2 \cos \left(\theta _5\right) \sqrt{A_{10}}
 \nonumber \\
A_{25} &=& -\frac{J}{4}+t+\frac{2 U}{3}+\frac{7 W}{3}+\frac{1}{12} \cos \left(\theta _5\right) \sqrt{A_{10}}-\frac{\sin \left(\theta _5\right) \sqrt{A_{10}}}{4 \sqrt{3}}
 \nonumber \\
A_{26} &=& -\frac{J}{4}+t+\frac{2 U}{3}+\frac{7 W}{3}+\frac{1}{12} \cos \left(\theta _5\right) \sqrt{A_{10}}+\frac{\sin \left(\theta _5\right) \sqrt{A_{10}}}{4 \sqrt{3}}
 \nonumber \\
%\eeq \newpage \beq
\small
\theta _1 &=& \frac{1}{3} \cos ^{-1}\left(\frac{\left(9 J^2+6 (9 t+4 U-4 W) J+8 \left(36 t^2+9 (U-W) t+2 (U-W)^2\right)\right) (3 J+4 U-4 W)}{A_1^{3/2}}\right)
 \nonumber \\
\theta _2 &=& \frac{1}{3} \cos ^{-1}\left(\frac{192 \sqrt{3} t^2 (3 J+4 U-4 W)}{A_2^{3/2}}\right)
 \nonumber \\
\theta _3 &=& \frac{1}{3} \cos ^{-1}\left(-\frac{\left(9 J^2+24 (U-W) J+16 \left((U-W)^2-36 t^2\right)\right) (3 J+4 U-4 W)}{A_3^{3/2}}\right)
 \nonumber \\
\theta _4 &=& \frac{1}{3} \cos ^{-1}\left(\frac{\left(9 J^2+24 (U-W) J+16 \left((U-W)^2-36 t^2\right)\right) (3 J+4 U-4 W)}{A_3^{3/2}}\right)
 \nonumber \\
\theta _5 &=& \frac{1}{3} \cos ^{-1}\left(\frac{(3 J+4 U-4 W) \left(9 J^2-6 (9 t-4 U+4 W) J+8 \left(36 t^2-9 (U-W) t+2 (U-W)^2\right)\right)}{A_{10}^{3/2}}\right)
\nonumber \eeq 
%\end{document}


==> triangle_abbreviations.tex <==
%\pagestyle{empty}
%\input{/home/schumann/TEX/mycommands}
%\begin{document}
\parindent0cm
\subsection*{ List of abbreviations }
\beq 
A_1 &=& 9 J^2+24 (U-W) J+16 \left(27 t^2+(U-W)^2\right)
 \nonumber \\
A_2 &=& 9 J^2+24 (t+U-W) J+16 \left(9 t^2+2 (U-W) t+(U-W)^2\right)
 \nonumber \\
A_3 &=& 9 J^2+24 (2 t+U-W) J+16 \left(36 t^2+4 (U-W) t+(U-W)^2\right)
 \nonumber \\
A_4 &=& 9 J^2-24 (t-U+W) J+16 \left(9 t^2-2 (U-W) t+(U-W)^2\right)
 \nonumber \\
A_5 &=& 9 J^2-24 (2 t-U+W) J+16 \left(36 t^2-4 (U-W) t+(U-W)^2\right)
 \nonumber \\
A_6 &=& -\frac{J}{4}+\frac{2 U}{3}+\frac{7 W}{3}-\frac{1}{6} \cos \left(\theta _1\right) \sqrt{A_1}
 \nonumber \\
A_7 &=& 3 J-8 U-28 W+2 \cos \left(\theta _1\right) \sqrt{A_1}
 \nonumber \\
A_8 &=& -\frac{J}{4}+\frac{2 U}{3}+\frac{7 W}{3}+\frac{1}{12} \left(\cos \left(\theta _1\right)-\sqrt{3} \sin \left(\theta _1\right)\right) \sqrt{A_1}
 \nonumber \\
A_9 &=& \frac{1}{3} \left(-\frac{3 J}{4}+2 U+7 W\right)+\frac{1}{12} \left(\cos \left(\theta _1\right)-\sqrt{3} \sin \left(\theta _1\right)\right) \sqrt{A_1}
 \nonumber \\
A_{10} &=& -\frac{J}{4}+\frac{2 U}{3}+\frac{7 W}{3}+\frac{1}{12} \left(\cos \left(\theta _1\right)+\sqrt{3} \sin \left(\theta _1\right)\right) \sqrt{A_1}
 \nonumber \\
A_{11} &=& \frac{1}{3} \left(-\frac{3 J}{4}+2 U+7 W\right)+\frac{1}{12} \left(\cos \left(\theta _1\right)+\sqrt{3} \sin \left(\theta _1\right)\right) \sqrt{A_1}
 \nonumber \\
%\eeq \newpage \beq
\theta _1 &=& \frac{1}{3} \cos ^{-1}\left(\frac{(3 J+4 U-4 W)^3}{A_1^{3/2}}\right)
\nonumber \eeq 
%\end{document}

